Continual Learning in Open-vocabulary Classification with Complementary Memory Systems

We introduce a method for flexible and efficient continual learning in open-vocabulary image classification, drawing inspiration from the complementary learning systems observed in human cognition. Specifically, we propose to combine predictions from a CLIP zero-shot model and the exemplar-based model, using the zero-shot estimated probability that a sample's class is within the exemplar classes. We also propose a "tree probe" method, an adaption of lazy learning principles, which enables fast learning from new examples with competitive accuracy to batch-trained linear models. We test in data incremental, class incremental, and task incremental settings, as well as ability to perform flexible inference on varying subsets of zero-shot and learned categories. Our proposed method achieves a good balance of learning speed, target task effectiveness, and zero-shot effectiveness. Code will be available at https://github.com/jessemelpolio/TreeProbe.

==> figures_latex/ablation_plots.tex <==
\begin{figure}[!htb]
 \centering
 \begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figures/ablation_plots.pdf}
\caption{(a) {\bf Left}: comparison of different KNN prediction variants in {\tt KNN} and \tp. for target and zero-shot tasks. Performances are averaged over all stages. (b) {\bf Right}: comparison of different fuse operations.}
\label{fig:ablation_plot}
\end{minipage}
\end{figure}

==> figures_latex/flexible_inference.tex <==
\begin{figure}[!htb]
 \centering
 \begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figures/flexible_inference.pdf}
\caption{}
\label{fig:flexible_inference}
\end{minipage}
\end{figure}

==> figures_latex/incremental_plot.tex <==
\begin{figure}[!htb]
 \centering
 \begin{minipage}{\textwidth}
% \includegraphics[width=\linewidth]{figures/incremental_plot.pdf}
\includegraphics[width=\linewidth]{figures/OWCL_main_results.pdf}
\caption{Results of various methods. ZS: zero-shot; FT: fine-tune; Exem. Only: only using exemplar-based prediction without considering zero-shot model prediction. (a) Average data incremental results across eight target tasks; (b) Average class incremental results across eight target tasks; (c) Task incremental results on target tasks; (d) Average zero-shot task results across all stages on different continual learning scenarios; (e) Results of flexible inference; (f) Comparison of different fuse operations. Note: for figures (a-d), performances are normalized relative to \czs\ performances on both target and zero-shot tasks. \zhen{Modification ideas after discussion: reorganize (f) to compare AIM and AVG side by side; rotate (d);}
% Dashed red lines in figures (a-c) represent the CLIP results.
% \derek{Can we make memory only --> exemplar only? Add dashed line at 100\% for a,b,c?  Can we put significance bars on (f) and (g)? } \zhen{Finished, except for the significance bar. Update later.}
\label{fig:incremental_plot}
}
\end{minipage}
% \vspace{-5mm}
\end{figure}

% \vspace{-7pt}

==> figures_latex/memory_prediction.tex <==
\begin{figure}[!htb]
 \centering
 \begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figures/memory_prediction.pdf}
\caption{}
\label{fig:memory_prediction}
\end{minipage}
\end{figure}

==> sections/3method.tex <==
\section{Method}
\vspace{-7pt}
\input{figures_latex/main_diagram}
Our approach is inspired from complimentary learning systems~\cite{cls_oreilley_2014}. CLS suggests that the human brain comprises two complementary subsystems: a rapid learning system and a slow learning system, which together facilitate efficient memory storage, retrieval, and generalization. The rapid learning system forms new memories and associations quickly, allowing for the storage of unique and episodic information. The slow learning system is responsible for the gradual extraction of general knowledge and regularities across experiences. The interplay between these two complementary systems enables the brain to achieve a balance between rapid encoding of novel information and the gradual generalization of knowledge. 

% In analogy to CLS, our model consists of two modules implementing the two systems: a base image encoder from CLIP which is extensively trained on large-scale data resembling the slow learning system, and an memory module storing extractions of images and annotations, functioning as the rapid learning system. We introduce these two modules in detail in the following along with the fuse operations to continually improve performances for learned classes while maintaining performances on zero-shot classes.

Analogous to CLS, our model comprises two modules: a CLIP-based base image encoder as the slow learning system, and a memory model storing extractions of images and annotations for rapid learning. We expect both modules to generate individual predictions and then fuse the outputs. In the following,  we detail these modules and their fusion operations, aimed at enhancing performance for learned classes while maintaining zero-shot classification performance. 

% We want to build an open-world classification model incorporating complementary learning systems. To this end, in addition to a base network that ensures the zero-shot ability to classify images, another core is a memory module storing instance-wise information. Essentially, the memory module makes instance-based predictions based on the input. To combine with the base network prediction, we devise several variants of fuse operations. The final classification label is given by taking the $\arg\max$ of the similarities between the output embedding with target class embeddings. 


\subsection{Open-vocabulary image classification}
\label{sec:open_voc_cls}
\vspace{-5pt}

% Meeting note with Derek: [define OVC, explain classification setting, explain in 3.2 how clip achieves open-world classification. In 3.3, explain better what we want to achieve: learn from new instances asap. Trying to catch batch based learning. Then explain linear probe has better performance compared to KNN and tree probe trying to catch constant time training. Mention LWR in 3.3 and state the drawback of it in evaluation. In Sec. 3.4, clearly explain we want clasisfication in exem set, if not in, then non-exemplar prediction. We need to be able to make prediction using a combination of .. give examples or even illustrate it.]

Image classification tasks in machine learning can be broadly bifurcated into {\bf closed-set} and {\bf open-vocabulary} scenarios. In closed-set classification, the model is trained on a finite set of known classes, and the goal is to classify new instances into one of these predefined categories. This paradigm, however, is incapable of recognizing or accommodating classes outside of the original training set. On the other hand, open-vocabulary classification allows for a more dynamic setting in which the set of classes can be defined at inference time. This flexibility introduces new challenges but enables the same model to more easily extend or blend its learned concepts and categories.  Open-vocabulary classification is typically enabled by learning a mapping from a text label to a classification vector, e.g. using a language model as in CLIP~\cite{clip}.


%The class set is not fixed and can expand or be defined at inference time, necessitating the model's capability to adjust to novel classes unseen during initial training. This flexibility to perform inference on a custom set of target classes

%Although this flexibility introduces additional challenges, it more accurately reflects real-world situations where new data categories may emerge.

At inference time, both closed-set and open-vocabulary classification involve choosing the most probable class $y_i$ from a candidate class set $Y$ given an input image $I$. We can postulate a function $f$ that maps $I$ to an embedding vector $e_I$, represented as $e_I= f(I)$.
% \begin{equation}
% e_I = f(I).
% \end{equation}
Additionally, a per-class weight vector $w_i$ is required to map $e_I$ to a corresponding class logit $l_i$ via an inner product, resulting in $l_i= w_i\cdot e_I$.
% \begin{equation}
% l_i= w_i\cdot e_I.
% \end{equation}
These weight vectors can either be learned or contextually provided. A softmax function is subsequently used to convert logits into probabilities: $p(y=y_i | I) = \frac{\exp(l_i)}{\sum_{j=1}^{n} \exp(l_j)}, \quad i = 1, \dots, n$ where $n$ is the number of classes. 
% \begin{equation}
% p(y=y_i | I) = \frac{\exp(l_i)}{\sum_{j=1}^{n} \exp(l_j)}, \quad i = 1, \dots, n.
% \end{equation}
The model finally yields the label $\hat{y}$ with the highest probability: $\hat{y} = \arg\max_{i} p(y=y_i | I).$
% \begin{equation}
% \hat{y} = \arg\max_{i} p(y=y_i | I). \label{eq:argmax}
% \end{equation}



% In the {\bf closed-set classification} scenario, the model is required to map an input image to a predefined set of known classes. Given an input image $I$, the model $f$ computes a set of logits $l$ for each of the $n$ possible classes. The logits represent the unnormalized log probabilities for each class:
% \begin{equation}
%     l = f(I) = [l_1, l_2, \dots, l_n]
% \end{equation}

% To obtain the probability distribution over the classes, we apply the softmax function to the logits: 
% \begin{equation}
%     p(y=y_i | I) = \frac{\exp(l_i)}{\sum_{j=1}^{n} \exp(l_j)}, \quad i = 1, \dots, n,
% \end{equation}
% where $y_i$ is the $i$-th label in the label set $\mathbf{C}$.

% The model predicts the label $\hat{y}$ with the highest probability: 
% \begin{equation}
%     \hat{y} = \arg\max_{i} p(y=y_i | I).
% \end{equation}
% We can use $\hat{y}$ to index the text label as well: $l(\hat(y))$.


\subsection{Slow learning system: zero-shot model}
\vspace{-5pt}
Artificial neural networks, as exemplified by foundational models such as CLIP~\cite{clip}, epitomize slow learning systems. Such networks learn iteratively, adjusting weights over multiple training epochs, aggregating over training data and developing increasingly abstract representations with increasing network depth. 
% This methodology has demonstrated effectiveness across diverse applications. 
Our approach leverages the CLIP image encoder as a slow learning mechanism due to its training on a massive image-text dataset and its ability for open-vocabulary classification by comparing image encodings to text encodings. We maintain fixed CLIP encoders throughout our project, since fine-tuning degrades the model's breadth of applicability.
%the original representation and may introduce forgetting.

Let denote the image encoder as $f_{\text{img}}$ and the text encoder as $f_{\text{txt}}$. Upon receiving an input image $I$ and a collection of textual labels $T = {t_1, t_2, \dots, t_n}$, the CLIP model maps $I$ and $T$ to their respective image and text embeddings, $e_I$ and $e_{t_i}$, represented as $e_I = f_{\text{img}}(I),  e_{t_i} = f_{\text{txt}}(t_i)$.

% \begin{equation}
% e_I = f_{\text{img}}(I), \quad e_{t_i} = f_{\text{txt}}(t_i).
% \end{equation}

Here, $e_{t_i}$ serves a role analogous to the weight vector $w_i$ from the previously defined classification model. The model computes logits for each class as cosine similarity between the image and text label, weighted by temperature $\tau$ (=100 in CLIP): $s(e_I, e_{t_i}) = \tau \cdot \frac{e_I \cdot e_{t_i}}{|e_I||e_{t_i}|}$, $i = 1, \dots, n.$
% \begin{equation}
% s(e_I, e_{t_i}) = \tau \cdot \frac{e_I \cdot e_{t_i}}{|e_I||e_{t_i}|}, \quad i = 1, \dots, n,
% \end{equation}
%The scores are 
Thus, cosine similarity substitutes for the inner product operation prevalent in closed-set models, and  the model applies a softmax function %parameterized by a temperature $\tau$ (=100 in CLIP), 
to transform logits into probabilities and selects  label $\hat{y}$ with highest probability, as in Sec~\ref{sec:open_voc_cls}. 
% \begin{equation}
% p_z(y=y_i|e_I) = \frac{\exp{( s(e_I, e_{t_i}))}}{\sum_{j=1}^{n} \exp{( s(e_I, e_{t_j}))}}.
% \end{equation}
%Finally, the model selects the label $\hat{y}$ corresponding to the highest probability, mirroring the decision-making process described in Sec~\ref{sec:open_voc_cls}. 

% Another way to yield a prediction is to produce an embedding, in this case, $\mathbf{v}_{\rm{mem}} = e_I$.

% \begin{equation}
% \hat{y} = \arg\max_{i} p_z(y=y_i|e_I).
% \end{equation}




% As described in Sec.~\ref{sec:open_voc_cls}, the embedding vector encoded by the CLIP image encoder can be used to compute similarities with target labels and perform open-vocabulary classification. When turning into the probabilistic format, the probability of the vector $\mathbf{v}_{\text{zs}}$ being label $y_i$ is:
% \begin{equation}
% p_z(y=y_i|\mathbf{v}_{\text{zs}}) = \frac{\exp{( \tau \cdot s(\mathbf{v}_{\text{zs}}, e_{t_i}))}}{\sum_{j=1}^{n} \exp{(\tau \cdot s(\mathbf{v}_{\text{zs}}, e_{t_j}))}}.
% \end{equation}


\subsection{Rapid learning system: exemplar-based memory model}
\label{sec:memory_prediction_approaches}
\vspace{-5pt}

For the rapid learning system, given one or more exemplars (image-label pairs), our goal is to maximize classification performance  with minimal training and acceptable inference time. 
%To harness the potential of the exemplar set, we explore two line of approaches for prediction and adaptation: 
We consider two approaches: instance-based and model-based prediction. Instance-based prediction leverages the exemplar set directly by retrieving and comparing samples. Model-based prediction seeks to capture the underlying structure of the data through a parameterized model. 

Our memory module $M$ stores encoded image embeddings along with their text labels $T$. Each entry in the memory can be denoted by $M_j=\{e_{I_j}, t_j\}$ where $j$ represents the entry index, $e_{I_j}$ represents the image embedding of $I_j$, and $t_j$ is the corresponding label. %To correlate with the concepts in a retrieval system, throughout the paper, we call: the input embedding $e_I$ as the {\it query}; $e_{I_j}$ of $M_j$ as the \textit{key}; and $t_j$ as the \textit{value}. 
% It is convenient to convert $t_j$ to the text embedding by: $e_{t_j}=f_{\text{txt}}(t_j)$. The memory module can represent a prediction as the probabilities of each target class  $p_e(y=y_i|e_I)$, or as a label embedding vector  $\mathbf{v}_{\text{mem}}$ similar to  RAC~\cite{rac}.
%make predictions for an input by giving the probability of being one of the target classes denoted by $p_e(y=y_i|e_I)$, or condensing the values to a memory embedding $\mathbf{v}_{\text{mem}}$ as similarly done in RAC~\cite{??}. 
%We define how to compute both forms for all proposed methods.
% In the following, we will delve into the details of both, highlighting their unique characteristics and strengths in the context of a rapid learning system. 

% \input{figures_latex/memory_prediction}
% \subsubsection{Instance-based prediction}


% \zhen{A diagram showing different IBP methods using the memory}

% \zhen{Weight can be a trick for any KNN methods, even for Majority vote. So the first prediction method should be KNN with majority vote solely. MV-KNN is for avg prob. fusion. Average KNN is for avg text fusion. Weighted MV-KNN, Weighted AVG-KNN can be an experiment to claim the effectiveness of weighting approach.}

% \zhen{While writing this part, we should start with how to produce the most possible label, aka, probabilities. Then in the next part, we would detail how to avg with text vectors. }

% Our memory module $M$ stores encoded image embeddings of samples in the exemplar set $\mathbf{E}$ along with their textual labels $T$. \zhen{Compare with rehearsal based approaches for continual learning. State that the storage of each entry is much smaller compared to them} Let $M_j=\{e_{I_j}, t_j\}$ denote the $j$-th entry in the memory and the memory contains in total $|M|$ entries. For simplicity, we call $e_{I_j}$ of $M_j$ as the \textit{key} and $t_j$ as the \textit{value}. 

{\bf KNN}: 
% We denote input image embedding $e_I$ as the query, $e_{I_j}$ of $M_j$ as the key; and label $t_j$ as the value. 
Given $e_I$, the KNN memory module finds its most similar $k$ entries in the memory through cosine similarities between $e_I$ and all $e_{I_j}$ in the memory. Let $\mathcal{N}_k(e_I)$ be the set of indices of the $k$ highest cosine similarity scores to $e_I$. KNN classification for $e_I$ can be performed by majority voting (\texttt{MV-KNN}) from the values:
$\hat{y} = \arg\max_{y} \sum_{j \in \mathcal{N}_k(e_I)} \mathds{1}(t_j = y).$
Here, $\mathds{1}(\cdot)$ is an indicator function. The probability of $e_I$ being label $y_i$ is 
$p_e(y=y_i|e_I) = \frac{\sum_{j \in \mathcal{N}_k(e_I)} \mathds{1}(t_j = y_i)}{k}$, and the label with maximum probability $\hat{y}$ is predicted. 

An alternative prediction approach is to produce a \emph{memory} embedding, denoted as $\mathbf{v}_{\text{mem}}$. For the retrieved instances, we encode the text labels into text embeddings using the CLIP text encoder. We could average the retrieved text embeddings (\texttt{AVG-KNN}):
$\mathbf{v}_{\text{mem}} = \frac{1}{k} \sum_{j \in \mathcal{N}_k(e_I)}  f_{\text{txt}}(t_j).$
Related to attention in transformers, we could also use a weighted average based on similarity (\texttt{WAVG-KNN}):
$\mathbf{v}_{\text{mem}} = \sum_{j \in \mathcal{N}_k(e_I)} \beta_{j} \cdot f_{\text{txt}}(t_j)$, where $\beta_{j} = \frac{\exp(s(e_I, e_{I_j}))}{\sum_{j' \in \mathcal{N}_k(e_I)} \exp(s(e_I, e_{I_{j'}}))}.$


KNN takes virtually no time to train ($\mathcal{O}(1)$), and reasonably fast retrieval is possible with optimized libraries and parallel computing. However, accuracy tends to be lower than model-based methods. %The major advantage of instance-based methods is fast adaptation, as the training time to incorporate a new exemplar is $\mathcal{O}(1)$, i.e. irrespective of the number of existing samples, since no model weights need to be tuned.  Inference time can range from $\mathcal{O}(\rm{log}~n)$ to $\mathcal{O}(n)$, depending on the retrieval mechanism, still efficient enough for many applications using optimized search libraries and parallel computing.

% \subsubsection{Model prediction}


{\bf Linear probe}: Model prediction offers an alternative approach, learning a fixed set of parameters that generalize patterns and learn the underlying structure of the data to maximize classification performance.  
%Even with well-trained encoders, instance-based predictors often under-perform model-based predictors with sufficient training data, since the models can tune feature weights and parameters for the classification task. 
%One limitation of instance-based prediction is the reduced accuracy of the assignment between queries and keys when the exemplar set expands exponentially. This issue is largely mitigated by utilizing the CLIP image encoder, as its pre-training objective function encourages a semantically meaningful and well-organized feature space. However, consolidating memory efficiently and compactly can further improve the performance and scalability of the instance-based prediction method. Model prediction offers an alternative approach to address these challenges by learning a fixed set of parameters that generalize patterns and learn the underlying structure of the data. 
%One design principle we follow for the model prediction methods is to maximize performance while minimizing the use of training resources.
Whenever new exemplars are added, the linear probe (\lp) method is to extract image embeddings and train linear classifiers on all accumulated exemplars. This relates to GDumb~\cite{prabhu_gdumb_eccv_2020}, a simple experience replay method that retrains models from scratch each time new data is received, but, to enable rapid learning, we do not retrain or fine-tune the encoder. 
%After storing the image embeddings and their labels, 
%As we store image embeddings and their labels directly in the exemplar set, we can train linear classifiers on these exemplars, similar to the linear probe approach. Learning a classifier is also similar to GDumb~\cite{??}, but we focus on learning linear classifiers instead of deeper networks to maintain a rapid learning speed. 
As in CLIP~\cite{radford_icml2021_clip}, we use the {\tt LogisticRegression} class from the sklearn library as the linear classifier. The output probability can be written as:
$p_e(y = y_i | e_I; \boldsymbol{\theta}) = \frac{\exp{(\boldsymbol{\theta}_{y_i}^T e_I)}}{\sum_{y_j\in \mathbf{C}} \exp{(\boldsymbol{\theta}_{y_j}^T e_I)}},$
where $\boldsymbol{\theta}_{y_i}$ represents the learned model parameters for label $y_i$. The memory embedding is the text embedding of the label $\hat{y}$ giving the maximum probability: $\mathbf{v}_{\text{mem}}=f_{\text{txt}}(t_{\hat{y}})$. 

Compared to KNN, the \lp\ model is much slower to train, $\mathcal{O}(n)$ for $n$ training samples assuming a constant number of epochs, which may be prohibitive when the model needs to be updated quickly based on few examples.  However, inference is faster than KNN, and classification accuracy tends to be higher.
%Compared to instance-based learning, the \lp\ model is much slower to train --- $\mathcal{O}(n)$ for $n$ training samples assuming a constant number of epochs --- but has faster inference, $\mathcal{O}(1)$, and, more importantly, tends to achieve higher accuracy than \knn\ for learned classes. This training time is a significant barrier in applications like active learning and retrieval with feedback, in which the model needs to be updated quickly based on a small number of examples.
% \zhen{Mention retraining the whole classifier for any new data.}

% One limitation of instance-based prediction is the assignment between query and keys becomes less accurate when the exemplar set expands exponentially. This is largely alleviated by utilizing CLIP image encoder since its pre-training objective function encourages the learned feature space to be semantically meaningful and well-organized. However, it still makes sense to consolidate memory in an efficient and compact manner to further improve the performance and scalability of the instance-based prediction method. model prediction offers an alternative approach to address some of these challenges. By learning a fixed set of parameters, model prediction seeks to generalize patterns and learn the underlying structure of the data through a set of optimized parameters. In the next, we introduce several model prediction methods with the targets to maximize performance yet minimize use of training resources. As we store image embeddings along with their labels directly in the exemplar set, we can train linear classifiers on those exemplars, in similar spirit to linear probe~\cite{??}. Learning a classifier is also similar to GDumb~\cite{??}, but we are only interested in learning linear classifiers instead of deeper networks to maintain a rapid learning speed. We follow CLIP to use the {\tt LogisticRegression} class in the sklearn library as the linear classifier. The output probability can be written as:
% $$p_e(y = y_i | e_I; \boldsymbol{\theta}) = \frac{\exp{(\boldsymbol{\theta}_{y_i}^T \mathbf{x}})}{\sum_{y_j\in \mathbf{C}} \exp{(\boldsymbol{\theta}_{y_j}^T \mathbf{x})}},
% $$
% assuming $\boldsymbol{\theta}_{y_i}$ is the learned model parameters for label $y_i$. We denote this approach using \texttt{LP}. 



% \hltext{red}{{\sc (Tree probe)}} As continual learning deals with potentially infinite data stream where distribution constantly shifts, it becomes increasingly difficult and inefficient to optimize a single linear classifier using all samples in the exemplar set. Therefore, given the whole exemplar set, we partition it into several clusters using KMeans. We train a single classifier within each cluster. Whenever new data arrives, we should rearrange original clusters and/or build new clusters. This requires training the classifiers where changes are made. To reduce work in training, inspired from tree-based clustering, we build the clusters by building a partition tree. Starting from a root node, we search the nearest leaf node for a new data point and fit it in that node \emph{iff.} the node has not reached the pre-defined capacity $\mathcal{C}$ yet. Whenever a leaf node reaches the capacity, it splits \emph{two} children leaf nodes and turns into a non-leaf node. Its attached data points are distributed to its children using KMeans clustering with cluster number set as 2. After the tree is built, each leaf node is treated as a cluster and attached with a linear classifier. When a new data point is added to the tree, only the affected node requires retraining its classifier. Compared to the training complexity of $\mathcal{O}(n)$ by \texttt{LP}, this method only has $\mathcal{O}(1)$. \zhen{A better illustration Table is needed} To fully leverage the power of the ensemble of classifiers, we incorporate kNN to give the final output probabilities. First, we compute the centroid of each cluster and searches the closest classifier by matching the similarity between the centroids and $e_{I_j}$, where $j \in \mathcal{N}_k(e_I)$. Let $\mathcal{C}_{k}(e_I)$ be the set of closest classifiers from the $k$ retrievals and $c$ is the index, $\boldsymbol{\theta}^{c}_{y_j}$ is the learned parameters of the classifier $c$ for the $y_i$ class from the corresponding class set denoted by $\mathbf{C}_c$. Then, the output probability is calculated by averaging the output probabilities of each classifier in $\mathcal{C}_{k}(e_I)$:
% $$p_e(y = y_i | e_I; \mathcal{C}_{k}(e_I)) = \frac{1}{k} \sum_{c \in \mathcal{C}_{k}(e_I)} \frac{\exp{({\boldsymbol{\theta}^{c}_{y_i}}^T e_I)}}{\sum_{y_j\in \mathbf{C}} \exp{({\boldsymbol{\theta}^{c}_{y_j}}^T e_I)}}.$$

% \zhen{Add the definition of the whole target class set}

{\bf Tree probe}: In a continual learning setting, we would ideally have fast training time of KNN with the relatively good accuracy of $\lp$.  Dusting off the older literature, we take inspiration from the instance-based and lazy learning~\cite{Aggarwal2014Chapter6I}, particularly locally linear models~\cite{domeniconi_2002_adaptivesvm_lazy,Atkeson1997LocallyWeightedLearning}.  These methods classify a test sample by finding its $k$-nearest neighbors and applying a linear classifier trained on the neighbors.  This achieves $\mathcal{O}(1)$ training time but may be impractical for inference, since a new classifier may need to be trained for each test sample.  


Instead, we propose an approximation, building a clustering tree from the training data and training a linear classifier in each leaf node. Starting from a root node, we search for the nearest leaf node for a new data point and insert it if the node has not reached the predefined capacity $\psi$ (=10000 in our experiments). If a leaf node reaches capacity, it splits into two child nodes and becomes a non-leaf node. The attached data points are distributed to their children using KMeans clustering with two clusters. In experiments, when receiving new data, samples are added into the cluster tree one by one. 
Only classifiers in affected leaf node(s) need to be retrained.  When fixing the number of linear model training epochs and KMeans iterations, the complexity to incorporate a new exemplar in training is $\mathcal{O}(\log~n+\psi)$; the training time stays limited even when the total number of exemplars is very large. 

The simplest inference method would be to assign a test sample to a leaf node in the cluster tree and classify it within the corresponding linear model, but this may lead to non-smooth predictions for samples near the cluster boundaries.  In our experiments, we use an ensemble of the classifiers from leaf nodes corresponding to the $k$ nearest neighbors for prediction.  Experimentally, we find this gives a modest boost to performance with a slight increase in inference time.  
For each classifier $c$, $\boldsymbol{\theta}^{c}_{y_i}$ represents the learned parameters for class $y_i$ from the corresponding class set $\mathbf{C}_c$. The output probability is calculated by averaging the output probabilities of each classifier in $\mathcal{C}_{k}(e_I)$.

The memory embedding can be computed as the text embedding of the most likely label or the average text embedding for the most likely label of each classifier in the retrieval set, but we obtain the best performance using a similarity-weighted average:
$  \mathbf{v}_{\text{mem}} = \sum_{c \in \mathcal{C}_{k}(e_I)} \beta_{c} \cdot f_{\text{txt}}(\arg\max_{y_i \in \mathbf{C}_c} p(y = y_i | e_I; c)), $ where $ \beta_{c} = \frac{\exp(s(e_I, e_{I_c}))}{\sum_{c' \in \mathcal{C}_{k}(e_I)} \exp(s(e_I, e_{I_{c'}}))}.$

This method, denoted \tp, achieves similar accuracy to \lp\ in our continual learning experiments, but with much faster training time. 

%find the k-nearest neighbors of a test sample at inference time and train a linear classifier using only those examples.  We propose, instead to build a clustering tree and train a classifier in each leaf node.    

%In continual learning, dealing with potentially infinite data streams with shifting distributions can make it difficult and inefficient to optimize a single linear classifier using all samples in the exemplar set. Instead, we partition the exemplar set into clusters using KMeans and train a separate classifier within each cluster. As new data arrives, we rearrange existing clusters and/or create new ones, necessitating the retraining of classifiers affected by these changes.

%To reduce the training workload, we draw inspiration from tree-based clustering and build a partition tree. %Each leaf node is considered a cluster and has an associated linear classifier. 


%find the $k$ nearest neighbors to a test sample and use the ensemble of classifiers from corresponding leaf nodes for prediction.  
%To fully leverage the ensemble of classifiers, we incorporate kNN to provide the final output probabilities. We compute the centroid of each cluster and find the closest classifier by comparing the centroids and $e_{I_j}$, with $j \in \mathcal{N}_k(e_I)$. Let $\mathcal{C}_{k}(e_I)$ be the set of closest classifiers from the $k$ retrievals. 


% $$p_e(y = y_i | e_I; \mathcal{C}_{k}(e_I)) = \frac{1}{k} \sum_{c \in \mathcal{C}_{k}(e_I)} \frac{\exp{({\boldsymbol{\theta}^{c}_{y_i}}^T e_I)}}{\sum_{y_j\in \mathbf{C}_c} \exp{({\boldsymbol{\theta}^{c}_{y_j}}^T e_I)}}.$$ 


%is $\mathbf{v}_{\text{mem}}=f_{\text{txt}}(t_{\hat{y}})$ if we use {\tt MV-KNN}. 
%Likewise, for {\tt AVG-KNN}, the memory embedding is calculated as an average of the embeddings corresponding to the maximum probability class of each classifier in the retrieval set:
%\begin{equation}
%\mathbf{v}_{\text{mem}} = \frac{1}{k} \sum_{c \in \mathcal{C}_{k}(e_I)} f_{\text{txt}}(\arg\max_{y_i \in \mathbf{C}_c} p(y = y_i | e_I; c)).
%\end{equation}
%For {\tt WAVG-KNN}, the memory embedding is obtained by reweighting the maximum probability class embeddings of each classifier based on the similarities between the query and the keys:
% \begin{equation}



% Assuming there are $|\mathbf{u}|$ classifiers in total and the output probabilities of a classifier attached to the cluster indexed with $z=1, \cdots, |\mathbf{u}|$ are denoted with $p_e^{\mathbf{u}_{z}}$.


% Since different classifiers have different trained labels, it is not reasonable to directly average probabilities for all labels together. For the inference, we combine with instance-based prediction approaches introduced above by considering only the predictions of classifiers of each retrieval.



% Assume the set of classifiers as $\mathbf{C}$. The classifier with each retrieval is denoted as: $\mathbf{C}_j$ with $j \in \mathcal{N}_k(e_I)$. The label prediction for each classifier is $\hat{y}_{\mathbf{C}_j}$. We can also find the corresponding text label emebeddings as $f_{\text{txt}}(\hat{y}_{\mathbf{C}_j})$. Then, 
% \begin{itemize}
% \item For \texttt{MV-KNN}, the final label is: $\hat{y} = \arg\max{c} \sum_{j \in \mathcal{N}k(e_I)} \mathds{1}(\hat{y}{\mathbf{C}j} = c)$.
% \item For \texttt{AVG-KNN}, the final label is: $\hat{y} = \arg\max{c} \frac{1}{k} \sum_{j \in \mathcal{N}k(e_I)} f_{\text{txt}}(\hat{y}{\mathbf{C}j})$.
% \item For \texttt{WAVG-KNN}, the final label is: $\hat{y} = \arg\max{c} \sum{j \in \mathcal{N}k(e_I)} \beta{j} \cdot f_{\text{txt}}(\hat{y}{\mathbf{C}j})$, where $\beta{j} = \frac{\exp(s(e_I, e{I_j}))}{\sum_{j' \in \mathcal{N}k(e_I)} \exp(s(e_I, e{I_{j'}}))}$.
% \end{itemize}

% $\hat{y} = \arg\max{c} \sum_{j \in \mathcal{N}k(e_I)} \mathds{1}(\hat{y}{\mathbf{C}j} = c)$




% {\bf (Tree probe)} 

% model prediction methods assume that the data can be represented by a parameterized model, which is learned by optimizing the parameters to minimize some loss function over the training data. By constructing a compact representation, model models can efficiently adapt to new data, generalize to unseen samples, and provide a more interpretable understanding of the relationships between the inputs and outputs.

% In this subsubsection, we will explore the development of a model prediction module within the rapid learning system. This module will complement the instance-based prediction approach, offering a more versatile and adaptive learning mechanism. The model model's design and training will be guided by the exemplar set, and its performance will be compared and contrasted with the instance-based prediction method. This comparison will serve to elucidate the advantages and limitations of both approaches and contribute to the development of a more comprehensive rapid learning system.

% \zhen{Continue by writing linear probe approaches}
% \vspace{-10pt}

\subsection{Fusing predictions of the two models}
\label{sec:fuse_operation}
\vspace{-5pt}

We want to integrate predictions from the CLIP model and the exemplar-based memory model to retain both good open-vocabulary classification performance and high accuracy on exemplar classes. This can be tricky, especially when a subset of classes in the task are covered by the exemplar classes.

%A limitation of the memory module is its restriction to exemplar class predictions, despite higher accuracy than open-vocabulary classification with the CLIP image encoder. To enable non-exemplar predictions and improve exemplar class performance, we consider bridging the two systems. However, integrating predictions from an exemplar model and a zero-shot model poses a non-trivial challenge.

One way is to obtain an output embedding vector $\mathbf{v}_{\text{out}}$ by averaging the zero-shot embedding $e_I$ and memory embedding $\mathbf{v}_{\text{mem}}$:
\begin{equation}
\label{eq:out_mem}
    \mathbf{v}_{\text{out}} = \alpha \mathbf{v}_{\text{mem}} + (1- \alpha)  e_I.
\end{equation}

Then we follow the open-vocabulary classification pipeline introduced in Sec.~\ref{sec:open_voc_cls} to obtain the final label. In design, $\alpha = 0.5$ is natural since it reflects equal confidences on zero-shot prediction and memory prediction. This simple fuse operation is called average vector (\texttt{Avg-Emb}).

From the probabilistic perspective, given the target class set $\mathbf{C}_{t}$, alternatively we can average probabilities from $p_e$ and $p_z$. Similarly, the final probability is:
\begin{equation}
\label{eq:out_prob}
p(y=y_i|I)=\alpha p_e(y=y_i|I) + (1-\alpha)p_z(y=y_i|I).
\end{equation} 
Here $\alpha$ is also 0.5 and we term the fuse operation \texttt{Avg-Prob}. 

% Our model generates final classification results in closed-set fashion with per-class logits or open-vocabulary fashion using embedding vectors for cosine similarity computation. Memory module predictions are described in Sec.\ref{memory_prediction_approaches}.

% For query embedding combination, we apply softmax with temperature parameter $\tau$ over similarities from Eq.\ref{eq:clip_similarity_calculation}:
% \begin{equation}
% p_z(y=y_i|I) = \frac{\exp{( \tau \cdot s(e_I, e_{t_i}))}}{\sum_{j=1}^{n} \exp{(\tau \cdot s(e_I, e_{t_j}))}}.
% \end{equation}
% With $\tau=100$, the final probability for an instance $I$ being $y_i$ is:
% \begin{equation}
% p(y=y_i|I)=\alpha p_e(y=y_i|I) + (1-\alpha)p_z(y=y_i|I).
% \end{equation}
% $\alpha$, a hyper-parameter, balances memory module and zero-shot predictions. We choose 0.5 for equal importance and term the fuse operation \texttt{Avg-Prob}. 




% However, these two approaches can be problematic since they assume equal importances of the exemplar model and zero-shot model for \emph{all} samples. We observe that when a test sample's label is within the exemplar's domain, the exemplar model tends to be more accurate, while for labels outside this domain, the zero-shot model typically performs better. However, in instances where the label set is only partially covered by the exemplar labels, it is often unclear whether a test sample's label falls within the exemplar set. 

% To tackle this, we propose an adaptive weighting mechanism to estimate the likelihood of a test sample's label being in the exemplar set and balance the predictions of both models accordingly. To estimate the likelihood, we first divide the whole target label set into two subsets: exemplar label set $y \in\mathbf{C}_e$ and non-exemplar label set $y\notin \mathbf{C}_{e}$. Then, we sum the probabilities over the two label sets and treat the sum as the likelihoods: $p(y\in\mathbf{C}_e|I) \propto \sum_{i \in \mathbf{C}_e} p_z(y=y_i|x)$ and $ p(y\notin\mathbf{C}_e|I) \propto \sum_{i \notin \mathbf{C}_e} p_z(y=y_i|x)= 1-p(y_i\in\mathbf{C}_e|I).$ Our key idea is to utilize zero-shot prediction as the confidence to decide whether a sample is in exemplar label set or not. We call this technique as adaptive instance marginalization ({\tt AIM}).

% Eq.~\ref{eq:out_mem} and Eq.~\ref{eq:out_prob} can be modified by replacing $\alpha$ with $p(y\in\mathbf{C}_e|I)$ and $1-\alpha$ with $p(y\notin\mathbf{C}_e|I)$. We further tweak Eq.~\ref{eq:out_prob} by combining zero-shot and memory predictions to capitalize on the strengths of both approaches for exemplar classes. In this case, Eq.~\ref{eq:out_prob} is substituted by:
% \begin{equation}
%     p(y=y_i|I)=p(y\in\mathbf{C}_e|I) \frac{p_z(y=y_i|I)p_e(y=y_i|I)}{\sum_{j\in \mathbf{C}_e} p_z(y=y_j|I) p_e(y=y_j|I)} + p(y \notin \mathbf{C}_e|I) p_z(y=y_i|I).
% \end{equation}


The \texttt{Avg-Emb} and \texttt{Avg-Prob} approaches presume equivalent influence of the exemplar and zero-shot models for all samples. This presumption does not hold when a test sample's label falls within the exemplar's domain, where the exemplar model is typically more accurate, or outside of this domain, where the zero-shot model tends to outperform.

Addressing this issue, we devise an adaptive weighting mechanism, named {\bf A}daptive {\bf I}nstance {\bf M}arginalization (\texttt{\bf{AIM}}), that estimates the likelihood of a test sample's label being in the exemplar set and balances the predictions from both models accordingly. The target label set is divided into exemplar $y \in\mathbf{C}_e$ and non-exemplar $y\notin \mathbf{C}_{e}$ subsets. The likelihoods $p(y\in\mathbf{C}_e|I)$ and $p(y\notin\mathbf{C}_e|I)$ are obtained by summing the probabilities over these subsets, with the zero-shot prediction providing a confidence metric for label set classification. Namely, $p(y\in\mathbf{C}_e|I) \propto \sum_{i \in \mathbf{C}_e} p_z(y=y_i|x)$ and $ p(y\notin\mathbf{C}_e|I) \propto \sum_{i \notin \mathbf{C}_e} p_z(y=y_i|x)= 1-p(y_i\in\mathbf{C}_e|I).$

To incorporate this, we revise Eq.~\ref{eq:out_mem} and Eq.~\ref{eq:out_prob}, replacing $\alpha$ with $p(y\in\mathbf{C}_e|I)$, resulting in two variants of fuse operations, namely {\tt AIM-Emb} and {\tt AIM-Prob}. This adaptive mechanism effectively capitalizes on the strengths of both prediction approaches, improving overall performance.

Since zero-shot predictions also have reasonable accuracies over exemplar classes, we also incorporate them with memory predictions for {\tt AIM-Prob}:
\begin{equation}
\label{eq:aim}
    p(y=y_i|I)=p(y\in\mathbf{C}_e|I) \frac{p_z(y=y_i|I)p_e(y=y_i|I)}{\sum_{j\in \mathbf{C}_e} p_z(y=y_j|I) p_e(y=y_j|I)} + p(y \notin \mathbf{C}_e|I) p_z(y=y_i|I).
\end{equation}
This induces a slight performance improvement. 

% Furthermore, for {\tt AIM-Prob}, we modify Eq.~\ref{eq:out_prob} to combine zero-shot and memory predictions for exemplar classes:
% \begin{equation}
% \label{eq:aim}
%     p(y=y_i|I)=p(y\in\mathbf{C}_e|I) \frac{p_z(y=y_i|I)p_e(y=y_i|I)}{\sum_{j\in \mathbf{C}_e} p_z(y=y_j|I) p_e(y=y_j|I)} + p(y \notin \mathbf{C}_e|I) p_z(y=y_i|I).
% \end{equation}
% This adaptive mechanism effectively capitalizes on the strengths of both approaches, improving overall performance.



% the posterior probability $p(y=y_i|I, y_i \in \mathbf{C}_e)$ is performed by:
% \begin{equation}
%     p(y=y_i|I, y \in \mathbf{C}_e)=p(y_i\in\mathbf{C}_e|I) \frac{p_z(y=y_i|I)p_e(y=y_i|I)}{\sum_{j\in \mathbf{C}_e} p_z(y=y_j|I) p_e(y=y_j|I)}.
% \end{equation}

% For non-exemplar classes, we rely on solely the zero-shot prediction:
% \begin{equation}
%     p(y=y_i|I, y_i \notin \mathbf{C}_e) = p(y_i \notin \mathbf{C}_e|I) \frac{p_z(y=y_i|I)}{\sum_{j \notin \mathbf{C}_e} p_z(y=y_j|I)},
% \end{equation} where $p(y_i\notin\mathbf{C}_e|I) \propto \sum_{i \notin \mathbf{C}_e} p_z(y=y_i|x)= 1-p(y_i\in\mathbf{C}_e|I)$.

% Writing the two equations together, the final probability of instance $I$ being label $y_i$ is:
% \begin{align}
%     p(y=y_i|I) = p(y=y_i|I, y_i \in \mathbf{C}_e) + p(y=y_i|I, y_i \notin \mathbf{C}_e).
% \end{align}

% Through this adaptive weighting mechanism, we effectively utilize predictions from both models to enhance the performance. This variant is called \texttt{}


% \subsubsection{new fuse}
% Integrating predictions from an exemplar model and a zero-shot model poses a challenge. When a test sample's label is within the exemplar's domain, the exemplar model tends to be more accurate, while for labels outside this domain, the zero-shot model typically performs better. However, in instances where the label set is only partially covered by the exemplar labels, it is often unclear whether a test sample's label falls within the exemplar set. To tackle this, we propose an adaptive weighting mechanism to estimate the likelihood of a test sample's label being in the exemplar set and balance the predictions of both models accordingly.

% We initially experimented with two straightforward approaches: Average Vector (\texttt{Avg-Emb}) and Average Probability (\texttt{Avg-Prob}). In \texttt{Avg-Emb}, the output embedding vector $\mathbf{v}_{\text{out}}$ is obtained by averaging the zero-shot embedding $\mathbf{v}_{\text{zs}}$ and memory embedding $\mathbf{v}_{\text{mem}}$. In \texttt{Avg-Prob}, we average probabilities from $p_e$ and $p_z$. However, these methods did not perform optimally, leading us to explore the adaptive weighting mechanism.

% For exemplar classes, we combine zero-shot and memory predictions:
% \begin{equation}
%     p(y=y_i|I, y_i \in \mathbf{C}_e)=p(y_i\in\mathbf{C}_e|I) \frac{p_z(y=y_i|I)p_e(y=y_i|I)}{\sum_{j\in \mathbf{C}_e} p_z(y=y_j|I) p_e(y=y_j|I)}.
% \end{equation}

% For non-exemplar classes, we rely solely on the zero-shot prediction:
% \begin{equation}
%     p(y=y_i|I, y_i \notin \mathbf{C}_e) = p(y_i \notin \mathbf{C}_e|I) \frac{p_z(y=y_i|I)}{\sum_{j \notin \mathbf{C}_e} p_z(y=y_j|I)},
% \end{equation} where $p(y_i\notin\mathbf{C}_e|I) \propto \sum_{i \notin \mathbf{C}_e} p_z(y=y_i|x)= 1-p(y_i\in\mathbf{C}_e|I)$.

% The final probability of instance $I$ being label $y_i$ is then constructed as:
% \begin{align}
%     p(y=y_i|I) = p(y=y_i|I, y_i \in \mathbf{C}_e) + p(y=y_i|I, y_i \notin \mathbf{C}_e).
% \end{align}

% Through this adaptive weighting mechanism, we effectively utilize information from both types of classes, enhancing performance and capability to handle outliers.




% \zhen{It seems that the }

% With the CLIP framework, one can also generate feature vector combining both the memory prediction and the zero-shot prediction. By doing this, 


% {\bf (Average KNN)} The memory module can alternatively provide an memory embedding $\mathbf{v}_{\text{mem}}$ by condensing the $k$ retrievals since the embedding can be directly used to compute similarities with target text features. A simple method is to average over the values of the retrievals. This is infeasible when the values are text labels but we can encode them to CLIP text embeddings through $f_{\text{txt}}$. Mathematically, the whole procedure can be described as:
% $$\mathbf{v}_{\text{mem}} = \frac{1}{k} \sum_{j \in \mathcal{N}_k(e_I)}  f_{\text{txt}}(t_j).$$
% We call this method as average KNN (\texttt{AVG-KNN}).

% {\bf (Weighted KNN)} Given the query, key and value tuples, one can reweight values by the similarities between query and keys. This in nature is similar to the cross-attention mechanism if we apply softmax over the similarities. In math, the memory embedding is obtained by:
% $$\mathbf{v}_{\text{mem}} = \sum_{j \in \mathcal{N}_k(e_I)} \beta_{j} \cdot f_{\text{txt}}(t_j),$$
% where
% $$\beta_{j} = \frac{\exp(s(e_I, e_{I_j}))}{\sum_{j' \in \mathcal{N}_k(e_I)} \exp(s(e_I, e_{I_{j'}}))} .$$ We refer to this method as weighted KNN (\texttt{WAVG-KNN}). 

% Our model can produce the final classification result using either the closed-set fashion by generating per-class logits, or the open-vocabulary fashion by yielding an embedding vector that can be used to compute cosine similarities with text embeddings. The predictions of the memory module generated by the closed-set fashion is mentioned in Sec.~\ref{memory_prediction_approaches}. While combining the query embedding, we apply softmax function over the similarities derived in Eq.~\ref{eq:clip_similarity_calculation} with a temperature parameter $\tau$. Written in math:
% \begin{equation}
%     p_z(y=y_i|I) = \frac{\exp{( \tau \cdot s(e_I, e_{t_i}))}}{\sum_{j=1}^{n} \exp{(\tau \cdot s(e_I, e_{t_j}))}}.
% \end{equation} 
% We follow the implementation of CLIP to set the temperature parameter as 100. 

% The final probability of an instance $I$ being $y_i$ is:
% \begin{equation}
%     p(y=y_i|I)=\alpha p_e(y=y_i|I) + (1-\alpha)p_z(y=y_i|I).
% \end{equation}
% Here, $\alpha$ is a hyper-parameter representing the importance of the prediction made by the memory module to the final prediction. Since we regard equal importance of zero-shot prediction and memory prediction, we choose it as 0.5. We call this fuse operation as average probability (\texttt{Avg-Prob}).


% However, this approach can be problematic for outlier instances in the memory. Consider the case that $I$ is an outlier to the memory, the zero-shot prediction is more probably accurate. Therefore, for better performance, we should consider a per-sample weighting mechanism. From our experiments, with all training data available, memory module has a better accuracy compared to zero-shot performance. That is to say, if a sample belongs to exemplar classes, it is better to choose memory prediction, otherwise if it is an outlier, zero-shot prediction should be more preferable. We are motivated to treat exemplar classes and non-exemplar classes differently. 

==> sections/4experiment.tex <==
\section{Experimental Setup}
\label{sec:experiment}


\subsection{Implementation details}
% \vspace{-5pt}
% All our experiments are conducted on a PC with an RTX 3090 graphics card and an AMD Ryzen 9 5950X 16-Core CPU. Our code is implemented with the PyTorch framework~\cite{??}. We follow the code example from CLIP to set the regularization strength of {\tt LogisticRegression} class in sklearn as 0.316 and the maximum iteration is set to 5K. The capacity of each node for tree probe is chosen as 10K. We use FAISS~\cite{faiss} to implement the retrieval system for its superior speed in retrieving samples from large-scale exemplar sets and use the exact search for inner product (IndexFlatIP) as the index class since it reduces less randomness and yields slightly better performance. We report Top-1 accuracy to compare the performances of different models. We use the officially released ViT-B/32 checkpoint from CLIP as our memory model or zero-shot model. More details can be found in supplementary.


We conduct our experiments on a setup featuring an RTX 3090 GPU and an AMD Ryzen 9 5950X CPU, using PyTorch as our primary framework. We adhere to the CLIP code example, setting the sklearn {\tt LogisticRegression} regularization strength to 0.316 and the maximum iteration is set to 5K. Our tree probe's node capacity is set at 50K. For efficient and high-speed retrievals from large-scale exemplar sets, we leverage FAISS~\cite{faiss}, specifically using the IndexFlatIP class for its precision and performance. Model performances are gauged via Top-1 accuracy, with the officially released ViT-B/32 CLIP checkpoint serving as our memory or zero-shot model. We select $k=9$ based on hyperparameter sweep on the validation tasks. Additional details are provided in the supplementary materials.

% For KNN, we set $k=12$ for {\tt MV-KNN} and $k=6$ for other variants, based on hyperparameter tuning on the validation tasks. 


% \vspace{-7pt}
\subsection{Tasks}
% \vspace{-5pt}
% Include table of classification tasks

\zhen{In this paper, we assume that seen samples can be stored in the memory and are always accessible across learning phases. Most prior works assume that past data is non-accessible due to privacy concerns but we mainly consider the case that users agree to upload their own data to the server and request prompt response, where efficient incremental learning is more at demand.}
In this paper, we evaluate our system on target and zero-shot image classification tasks. A ``task'' is an assignment of an image from some distribution into a label from particular label set.  The exemplar model has received examples in the context of ``target'' tasks but not ``zero-shot'' tasks.  We utilize {\bf general tasks} such as ImageNet~\cite{ImageNet}, SUN397~\cite{sun397}, CIFAR100/10~\cite{cifar_100}, Caltech101~\cite{caltech101}, and {\bf fine-grained tasks} like EuroSAT~\cite{eurosat}, OxfordIIITPets~\cite{oxfordpets}, SVHN~\cite{SVHN}, DTD~\cite{dtd}, Flower102~\cite{flowers102}, FGVCAircraft~\cite{fgvc_aircraft}, StanfordCars~\cite{stanfordcars}, Food101~\cite{Food101}, Resisc45~\cite{Resisc45}, UCF101~\cite{UCF101}.

We report main results using target tasks  CIFAR100, SUN397, FGVCAircraft, EuroSAT, OxfordIIITPets, StanfordCars, Food101 and Flowers102 and zero-shot tasks ImageNet, UCF101, and DTD.  To avoid selection bias, we perform hyper-parameter searches using held out target tasks CIFAR10, SVHN, Resisc45 and zero-shot task Caltech101.
The supplemental materials contains more details for the tasks, including description of datasets, prompt templates, and zero-shot performance. 

%Hyper-parameter searches are conducted on target tasks CIFAR10, SVHN, and Resisc45, and a zero-shot task Caltech101. For main results, to mitigate hyperparameter selection bias, we adopt different tasks: CIFAR100, SUN397, FGVCAircraft, EuroSAT, OxfordIIITPets, StanfordCars, Food101 and Flowers102 as target tasks; and ImageNet, UCF101, and DTD as zero-shot tasks. This selection, comprising both general and fine-grained tasks, more thoroughly evaluates our model's zero-shot performance. More details including prompt templates and zero-shot performances on all tasks are provided in the supplementary materials.

% We treat classification on a single dataset as a classification task. 
% To evaluate our system, depending on whether the samples of a task are fed to the memory model, we split them into target tasks and zero-shot tasks.

% In this paper, the classification tasks we consider include {\bf general tasks}: ImageNet~\cite{ImageNet}, SUN397~\cite{sun397}, CIFAR100/10~\cite{cifar_100}, Caltech101~\cite{caltech101} and {\bf fine-grained tasks}: EuroSAT~\cite{eurosat}, OxfordIIITPets~\cite{oxfordpets}, SVHN~\cite{SVHN}, DTD~\cite{dtd}, Flower102~\cite{flowers102}, FGVCAircraft~\cite{fgvc_aircraft}, StanfordCars~\cite{stanfordcars}, Food101~\cite{??}, Resisc45~\cite{??}, UCF101~\cite{??}.

% For hyper-parameter search and ablation experiments, the target tasks include CIFAR10, SVHN and Resisc45, whereas the zero-shot task is Caltech101. To avoid concerns of the hyperparameter selection biased towards our approaches, for main results, we use different tasks: CIFAR100, SUN397, FGVCAircraft, EuroSAT, OxfordIIITPets, StanfordCars, Food101 and Flowers102 as target tasks; ImageNet, UCF101 and DTD as zero-shot tasks. To select tasks for zero-shot evaluation, we consider both general (e.g., ImageNet) and fine-grained tasks (e.g., DTD) to give a thorough evaluation of the model's ability in handling zero-shot tasks.

% More details are given in the supplementary materials.



\subsection{Evaluation scenarios}
% \vspace{-5pt}

We consider several continual learning scenarios for receiving data: 1) {\bf Data incremental}: A fraction of the training data, randomly sampled without enforcing class balance, is added in each stage; 2) {\bf Class incremental}: All training data for a randomly sampled subset of classes are added in each stage; 3) {\bf Task incremental}: All data for a single task, i.e. a dataset of examples assigned to a set of target labels, are added in each stage. 
Data incremental learning includes seven stages, each comprising 2\%, 4\%, 8\%, 16\%, 32\%, 64\%, and 100\% of task data respectively. Class incremental learning divides a task into five stages, each containing 20\% of classes. In task incremental learning, each task is considered a stage.
In data and class incremental experiments, models are built separately for each target task. A target task is fully evaluated if there is at least one training sample for that task, even if there are no training samples for some classes. In task incremental, one model is built spanning all of the accumulated labels in each stage.  In all cases, results are reported as the average accuracy of target tasks and of zero-shot tasks at each stage.
% , all normalized by baseline zero-shot accuracy.
% \input{figures_latex/data_scenarios}
 % \derek{Checking -- are performances of all zero-shot tasks averaged?}

% In the task incremental setting, after all training data for target tasks is received, we also evaluate each method's performance in several inference scenarios: \textbf{T} Target task; \textbf{Z} Zero-shot task; \textbf{U} Union of target task labels: in each task, the union of all labels is considered as valid predictions; \textbf{U-Z} Same as above, but a random sample of 100 labels from the zero-shot task are also added, and the average of target and zero-shot task performances are reported; \textbf{M} Mix of target task labels: randomly split the union of target labels into five splits, and average performance across splits is reported with 100 test samples per class; \textbf{M-Z} Same as above, but adding a random sample of 100 labels from the zero-shot task in each split. 

\noindent {\bf Flexible inference:}~In the task incremental setting, after all training data for target tasks is received, we also evaluate each method's performance in two inference scenarios: \textbf{U} Union of target task labels: in each task, the union of all labels is considered as valid predictions; \textbf{U-Z} Same as above, but a random sample of 100 labels from the zero-shot task are also added, and the average of target and zero-shot task performances are reported. These two inference scenarios evaluate the model's flexibility and robustness under different label splits. A more advanced method expects to have higher accuracies under these scenarios.




\section{Experimental Results}
% \vspace{-7pt}
In Sec.~\ref{sec:results_main}, we compare three forms of exemplar-based memory models.
% with and without fusion with the zero-shot model, using hyper-parameters selected using the validation tasks.  
We then present results of ablation experiments (Sec.~\ref{sec:results_ablation}), evaluating the methods of nearest neighbor blending and model fusion.  Next, we evaluate with larger zero-shot backbones (Sec.~\ref{sec:results_scaling}), and finally present results on long-tailed classification (Sec.~\ref{sec:results_long_tailed}).  

\subsection{Main Results}
\label{sec:results_main}
\vspace{-5pt}
%\subsubsection{Comparison under different evaluation scenarios}
% \zhen{We need to come up with a way to rule out comparisons with other approaches.}

% To our knowledge, there is limited work on continual learning aiming to address forgetting and maintain open-vocabulary classification capabilities. 

% \input{figures_latex/incremental_plot}
% \input{figures_latex/flexible_inference}

\input{figures_latex/fig2}

We compare performance of the three forms of exemplar-based models on target tasks, zero-shot tasks, mixes, and unions (Figs.~\ref{fig:incremental_plot}). We compare using only the exemplar models, in which zero-shot performance suffers, and fusing the zero-shot and exemplar-based models' predictions using the \texttt{AIM-Emb} method. We consider the CLIP zero-shot model as a baseline termed as \texttt{CLIP-ZS}.  We normalize the performances of different approaches with the \texttt{CLIP-ZS} to show the influence of learning, as \texttt{CLIP-ZS} is the starting point for all approaches. Ideally, target task performance would rise above 100\% (improved), while zero-shot performance would maintain near 100\% (no change).  

%Our fused model comprises a memory model and a zero-shot model. We would like our fused model to outperform the zero-shot model in target tasks and the memory model in zero-shot tasks. 
%We consider the zero-shot model as a baseline termed as \texttt{CLIP-ZS}. As introduced in Sec.~\ref{sec:memory_prediction_approaches}, we have three prediction approaches for the memory model, namely {\tt KNN}, \lp\ and \tp . Consequently, we have three variants for the fused model with different memory prediction approaches, namely {\tt KNN fused}, {\tt Linear probe fused} and {\tt Tree probe fused}. The comparison results of these approaches are illustrated in Fig.~\ref{??}. We normalize the performances of different approaches with the \texttt{CLIP-ZS} to show the influence of learning as \texttt{CLIP-ZS} is the starting point for all approaches. 

We are not aware of existing works that address continual learning in an open-vocabulary image classification setting, but WiSE-FT~\cite{WiSE-FT} can be easily modified to address this problem.  Initializing from a pre-trained model (image encoder and text embeddings for linear weights), such as CLIP, WiSE-FT fine-tunes the image encoder and/or linear model on the target data.  Then, the new weights are element-wise weighted-averaged with the original weights, with a blending parameter $\alpha$ (= 0.5 by default).  This method was proposed and evaluated as a way to maintain robustness to domain shift.
% , e.g. classifying both natural images and sketches of the target classes.  
To extend to continual learning, when new data is received, the linear model(s) for corresponding task(s) are tuned, and we replace the text embeddings for trained classes with the average ($\alpha=0.5$) of the original embedding and the trained weights.  This is similar to our \lp\ method and shares the disadvantage of time complexity to incorporate new data.

%One notable approach, WiSE-FT, initiates a linear classifier using CLIP text embeddings for target classes before undergoing fine-tuning. Upon completion, the fine-tuned weight is averaged with the zero-shot weight using a blending parameter $\alpha$ typically set to 0.5. This averaged classifier demonstrates resilience to domain shifts and often outperforms both standalone models. We view the averaging of classifier weights as a potential means to balance between zero-shot and target tasks. We adjust our \lp\ prediction method to facilitate this. For classes within the exemplar set, we average the weights from the beginning and end of the fine-tuning process for a target task. Conversely, for classes absent from the exemplar set, we directly employ the weights from the corresponding target class text embeddings. This ensemble classifier generates prediction logits for the target classes, with the label selected as the one with the maximum probability, as determined by softmax. We mark this method as \lp\ (WiSE-FT).


From Fig.~\ref{fig:incremental_plot}(a-c), \lp, \tp, and \texttt{WiSE-FT} outperform other methods across all stages. In the early stages of data and class incremental scenarios, the exemplar-based models cannot perform well on their own, due to limited data. However, with more data, these methods improve and eventually surpass \czs\ for target tasks. Yet, they perform very poorly in zero-shot tasks, as their reliance on exemplars provides limited information for non-exemplar classes, as depicted in Fig.~\ref{fig:incremental_plot}(d). \texttt{AIM} restores zero-shot performance across all exemplar models and scenarios.  

\texttt{WiSE-FT} performs well in the low-data regime of data incremental and class incremental scenarios for target tasks, but underperforms slightly in the high data regime of class incremental.  Also, its zero-shot performance falters in the task incremental scenario, since this scenario requires multiple incremental adjustments to the linear weights. \derek{fact check?}

Fig.~\ref{fig:incremental_plot}(e) shows non-normalized accuracies across models for various tasks. In U, T, and M tasks, exemplar-based models surpass the CLIP zero-shot model, highlighting their efficacy in learned categories tasks. However, their Z task performance significantly diminishes, indicating their limitations in unseen categories. With \texttt{AIM}, models' Z tasks performance remarkably improves, without impacting their U, T, and M tasks performance. This underscores \texttt{AIM}'s role in enhancing models' unseen categories handling while maintaining their learned tasks competence. WiSE-FT excels in T and M tasks but underperforms in Z and Z-involved tasks. \lp\ outperforms \tp\ in U and T, with other tasks being comparable. However, \tp\ is significantly more efficient, taking only 40 minutes to complete all stages in the task incremental setting, while \lp\ requires over 8 hours. Thus, \tp\, when fused with {\tt AIM}, provides the best balance between performance and efficiency, making it our most recommended approach.


% Though the performance of \tp is slightly inferior to \lp , \tp roughly requires only 40 mins to finish passing all stages in the task incremental setting but \lp usually needs over 10 hours when there are no other ongoing programs on the computer. 
% These findings highlight the effectiveness of model fusion for flexible inference and the trade-off between target task and zero-shot performance in memory-only approaches. 

% \zhen{time}


% \zhen{talk about flexible inference}


%\subsubsection{Flexible inference}

\input{figures_latex/fig3}

\subsubsection{Comparison to previous methods}
Most prior works are designed for closed-vocabulary continual classification tasks and cannot be directly applied to open-vocabulary continual learning. A recent work called ZSCL~\cite{ZSCL} explores a similar setting to us and is mainly evaluated under the task-incremental learning scenario. Since their method requires large compute to run, we mainly evaluate our approach under their evaluation protocols. To keep comparison fair, we utilized the same prompt ensemble technique, data split ratio and seed, backbone network (ViT-B/16), \emph{etc.} The result comparison is illustrated in Tab.~\ref{tab:comparison_to_zscl}. All results are taken from other ZSCL's paper except for ours. 

\input{tables/comparison_to_zscl}


\subsection{Ablation experiments}
\label{sec:results_ablation}
\vspace{-5pt}
For ablation experiments, we mainly consider the task incremental learning scenario, as incrementally incorporating data from each task is more challenging than inrementally receiving data mixed across tasks.  More results are in supplementary materials, including selection of $k$.

% {\bf Time analysis of memory prediction approaches}
% For the memory model, we would like to know the time analysis and characteristics of each prediction approach.

% \input{figures_latex/ablation_plots}

% \input{tables/knn}

\zhen{Instead of this variants of KNN experiments, probably we can try ablating the cluster size of TreeProbe as it is also relevant to the performance. We haven't done a thorough study about this before NeurIPS ddl and maybe we can find a better performance. }

\zhen{After discussion: Add two plots, one plot is ACC (y-axis) vs. Time (x-axis). Another plot is Num of samples in the memory (x-axis) vs. learning time (y-axis), maybe accuracy at the tail of each line.}

{\bf Comparison of variants of KNN prediction} In Sec.~\ref{sec:memory_prediction_approaches}, we describe three variants of KNN prediction approaches, namely {\tt MV-KNN}, {\tt AVG-KNN} and {\tt WAVG-KNN}. As \tp\ also involves the procedure of aggregating results from the $k$ nearest classifiers, we also experiment on the \tp\ approach. We report averaged accuracy for both target tasks and zero-shot tasks by averaging across all stages. In Fig.~\ref{fig:incremental_plot}(f), we see that {\tt MV-KNN} achieves highest average accuracy for KNN predictions, while {\tt WAVG-KNN} achieves highest for \tp\ prediction, though the differences are small. \derek{Are these differences significant?  We could simply the method and experiment section if discussion of these variants and corresponding results are moved to the supplemental materials.}

% \input{tables/fuse}

{\bf Comparison of variants of fuse operations} As delineated in Sec.~\ref{sec:fuse_operation}, we propose four fusion operations: {\tt Avg-Prob}, {\tt Avg-Emb}, {\tt AIM-Prob}, and {\tt AIM-Emb}. The {\tt AIM} fusion greatly outperforms unweighted average for both target and zero-shot tasks.  {\tt AIM-Emb} enables slightly better zero-shot performance than {\tt AIM-Prob} (53.7 vs. 51.04) with marginally lower target task performance (67.9 vs. 68.5), making it preferred overall. 

%Experimental results, averaged across stages and depicted in Fig.~\ref{fig:incremental_plot}(g), validate our choice of {\tt AIM-Emb} as the best-performing fusion operation. This selection is based on the superior performance of {\tt AIM} variants over {\tt Avg} ones, particularly noticeable in both target and zero-shot tasks. Despite {\tt AIM-Emb} showing marginally lower target performance compared to {\tt AIM-Prob}, it confers distinct advantages in zero-shot tasks. We thus employ {\tt AIM} for blending predictions from the zero-shot model and the memory model, averaging the embeddings to achieve overall enhanced performance.


% {\bf Selection of K in KNN} 


\subsection{Scaling to larger zero-shot models}
\label{sec:results_scaling}
\vspace{-5pt}
\input{tables/scaling}

Our main experiments use the CLIP ViT/B-32 model as our zero-shot model, but our approach can easily be adapted to other models. We experiment with the pretrained CLIP model ViT-L/14@336px, which boasts approximately 4x the capacity of ViT-B/32, and ViT-H/14\footnote{Checkpoint from \url{https://github.com/mlfoundations/open_clip}}, which is double the size of ViT-L/14@336px. We present our findings in Tab.~\ref{tab:scaling}. Performance increases for larger models, and \tp\ consistently outperforms \czs\ on the target tasks by large margins (roughly 25\% to 33\% relative reduction of error in each case) with nearly identical performance on the zero-shot tasks, demonstrating that our approach is beneficial for a wide range of zero-shot model sizes. 


\subsection{Evaluation on long-tailed classification}
\label{sec:results_long_tailed}
\vspace{-5pt}
\input{tables/long_tailed_classification}

In long-tailed classification, some test labels are rare or unobserved in training, so blending exemplar-based models with consolidated models can be beneficial, as shown by~\cite{rac}.  To accommodate this setting, we adjust our {\tt AIM-Emb} method by considering the 2/3 rarest labels as not being present in the exemplar set and the remainder as being present, for the purpose of calculating $\mathbf{v}_\text{out}$. In Tab.~\ref{tab:long_tailed_classification}, we present results on the Places365LT dataset~\cite{Places365LT}.  Our {\tt AIM-Emb} method with \lp\ and \tp\ outperform the zero-shot baseline.  We also compare to PaCo~\cite{PaCo} and RAC~\cite{rac}, which are specifically designed for long-tail classification.  PaCo incorporates learnable class centers to account for class imbalance in a contrastive learning approach.  RAC trains an image encoder that is augmented with label predictions from retrieved exemplars.  Although not specifically designed for long-tailed classification, our method performs similar to PaCo, but RAC performs best of all. 




%As shown in RAC~\cite{rac}, their framework has superior performance on long-tailed classification, demonstrating the retrieval procedure provides benefits to tail classes. Likewise, in addition to the continual learning settings, we explore the possibilities of extending our method for long-tailed classification. 
%Specifically, we note the zero-shot model's proficiency in distinguishing \emph{tail} classes, while the memory model exhibits superior accuracy for \emph{head} classes. Following this, we categorize classes into {tail} ($\mathbf{C}_{\rm{tail}}$) and {head} ($\mathbf{C}_{\rm{head}}$) based on their sample sizes, designating the bottom two-thirds as \emph{tail}. Then, in line with the {\tt AIM} approach, we amalgamate the zero-shot ($e_I$) and memory ($\mathbf{v}_{\text{mem}}$) embeddings, using the probability of a sample's affiliation to either the head or tail class, to produce the output embedding: $\mathbf{v}_{\text{out}} = p(y\in\mathbf{C}_{\rm{head}}|I) \mathbf{v}_{\text{mem}} + p(y\in\mathbf{C}_{\rm{tail}}|I) e_I$. 
%Here, $p(y\in\mathbf{C}_{\rm{head}}|I) \propto \sum_{i \in \mathbf{C}_{\rm{head}}} p_z(y=y_i|x)$ and $p(y\in\mathbf{C}_{\rm{tail}}|I) = 1 - p(y\in\mathbf{C}_{\rm{head}}|I)$.

%Accuracy on the Places365LT dataset~\cite{Places365LT} is presented in Tab.~\ref{tab:long_tailed_classification}. These results demonstrate that all three memory prediction approaches, when enhanced with {\tt AIM}, outperform their respective versions without {\tt AIM}.
%Our method performs similarly to PaCo~\cite{PaCo}, while RAC achieves higher accuracy. 
% thus validating its effectiveness. 
%Compared to recent works specifically designed for long-tailed recognition, our method performs similarly to PaCo~\cite{PaCo}, while RAC achieves moderately higher accuracy.


% Specifically, with the observation that zero-shot model excels at differentiating \emph{tail} classes compared to the memory model that gives more accurate prediction on \emph{head} classes, following the principle of the proposed {\tt AIM}, we bifurcate classes into \emph{tail} ($\mathbf{C}{\rm{tail}}$) and \emph{head} ($\mathbf{C}{\rm{head}}$) based on sample sizes, with the lower two-thirds constituting the former. We then fuse the zero-shot ($\mathbf{v}{\text{zs}}$) and memory ($\mathbf{v}{\text{mem}}$) embeddings according to the probabilities of samples falling into either head or tail classes, resulting in the output embedding $\mathbf{v}_{\text{out}}$:
% \begin{equation}
% \mathbf{v}_{\text{out}} = p(y\in\mathbf{C}_{\rm{head}}|I) \mathbf{v}_{\text{mem}} + p(y\in\mathbf{C}_{\rm{tail}}|I) \mathbf{v}_{\text{zs}}.
% \end{equation}
% This equation represents the weighted average of the memory and zero-shot embeddings, with weights determined by the class probabilities.

% \texttt{AIM} leverages the zero-shot estimation to discern whether a sample belongs to tail classes, integrating both the memory model and the CLIP zero-shot model. \texttt{LinProbe} and \texttt{TreeProbe} perform well on classes with plentiful samples, but their efficacy dwindles for tail classes due to limited training data. Conversely, the CLIP zero-shot model performs reasonably on tail classes but doesn't significantly improve for non-tail classes despite training data.

% To overcome these constraints, we bifurcate classes into \emph{tail} ($\mathbf{C}{\rm{tail}}$) and \emph{head} ($\mathbf{C}{\rm{head}}$) based on sample sizes, with the lower two-thirds constituting the former. We then fuse the zero-shot ($\mathbf{v}{\text{zs}}$) and memory ($\mathbf{v}{\text{mem}}$) embeddings, guided by the zero-shot probabilities of samples falling into either class, resulting in the output embedding $\mathbf{v}_{\text{out}}$:
% \begin{equation}
% \mathbf{v}{\text{out}} = p(y\in\mathbf{C}{\rm{head}}|I) \mathbf{v}{\text{mem}} + p(y\in\mathbf{C}{\rm{tail}}|I) \mathbf{v}_{\text{zs}}.
% \end{equation}
% This equation represents the weighted average of the memory and zero-shot embeddings, with weights determined by the class probabilities.

% Specifically, \texttt{AIM} provides a way to make the best of the rapid learning system and CLIP zero-shot model based on the zero-shot estimation of whether the sample belongs to the tail classes. \texttt{LinProbe} and \texttt{TreeProbe} in the rapid learning system can achieve a decent accuracy in classes with large amounts of samples, but their performance for tail classes may suffer from the lack of training samples. Meanwhile, CLIP zero-shot model can handle tail classes reasonably well, but its performance on non-tail classes would not further improves with the benefits brought by training data. Hence, we divide all classes into two parts based on their number of samples. 2/3 classes with smaller amount of samples are referred as \emph{tail} classes ($\mathbf{C}_{\rm{tail}}$), while the rest are referred as \emph{head} classes ($\mathbf{C}_{\rm{head}}$). Similar to Eq.~\ref{eq:aim}, we fuse the zero-shot embedding $\mathbf{v}_{\text{zs}}$ and memory embedding $\mathbf{v}_{\text{mem}}$ based on the zero-shot probability of the sample belonging to \emph{tail} classes and \emph{head} classes:
% $\mathbf{v}_{\text{out}}$ by averaging the zero-shot embedding $\mathbf{v}_{\text{zs}}$ and memory embedding $\mathbf{v}_{\text{mem}}$:
% \begin{equation}
%     \mathbf{v}_{\text{out}} = p(y\in\mathbf{C}_{\rm{head}}|I) \mathbf{v}_{\text{mem}} + p(y\in\mathbf{C}_{\rm{tail}}|I) \mathbf{v}_{\text{zs}}.
% \end{equation}

% \subsection{Baselines}

% We consider several baselines:
% \begin{itemize}
%     \item \texttt{CLIP-ZS}: as we leverage CLIP as the base network which enables open-vocabulary classification, while illustrating the performance gain brought by our approach, one natural baseline is the CLIP zero-shot performances on evaluated datasets.
%     \item \texttt{CLIP-LP}: we would also want to compare with the linear probe performances by training a linear classifier on extracted CLIP image features and their corresponding labels from the training data.
%     \item \texttt{CLIP-LP w/ ZS}: the naive linear probe model cannot evaluate performance on open-vocabulary classes unless combined with zero-shot confidences. To enable zero-shot task comparison, we further append the zero-shot probabilities of exclusive classes during evaluation. To obtain those probabilities, we apply softmax over cosine similarities between the query feature and target class features.
% \end{itemize}

    % \item \texttt{KNN}: the exemplar module standalone can produce instance-based predictions whereas the predictions are constrained in exemplar classes only. To maintain generality, this baseline 
    % \item \texttt{KNN w/ ZS}: similar to \texttt{CLIP-LP w/ ZS}, \texttt{KNN} can also combine with zero-shot predictions to give predictions on non-exemplar classes. Instead of giving probabilities for all target classes, we average the CLIP embedding with 




==> tables/ensemble_classifiers.tex <==
\begin{table}[ht]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Stage I} & \multicolumn{2}{c}{Stage II} & \multicolumn{2}{c}{Stage III} & \multicolumn{2}{c}{Stage IV} & \multicolumn{2}{c}{Stage V} & \multicolumn{2}{c}{Stage VI} & \multicolumn{2}{c}{Stage VII} & \multicolumn{2}{c}{Stage VIII} \\ \cline{2-17}
 & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot \\ \hline
\tp\ w/o ensem. cls. & 60.3 & 53.6 & 63.0 & 53.5 & 70.3 & 53.8 & 70.3 & 53.7 & 70.0 & 53.8 & 71.9 & 53.8 & 74.8 & 53.8 & 74.4 & 53.8  \\ \hline
\tp\ & 61.7 & 53.9 & 63.2 & 53.8 & 70.6 & 53.9 & 70.6 & 53.8 & 70.6 & 53.8 & 72.5 & 53.8 & 75.5 & 53.8 & 75.3 & 53.9 \\  \hline
\end{tabular}
\end{adjustbox}
\caption{Accuracies of \czs\ and \tp\ on target and zero-shot tasks with pretrained image encoders of different capacities.}
\label{tab:ensemble_classifiers}
\end{table}

==> tables/fuse.tex <==
% \begin{table}[ht]
% \centering
% % \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{l|cc|cc|cc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{2}{c}{Stage I (CIFAR10)} & \multicolumn{2}{c}{Stage II (SVHN)} & \multicolumn{2}{c}{Stage III (Resisc45)} \\ \cline{2-7}
%  & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot \\ \hline
% {\tt AVG-Prob} & 43.67 & 83.63 & 54.48 & 83.63 & 83.54 & 83.63 \\ 
% {\tt AVG-Emb} & 36.28 & 12.74 & 58.73 & 29.68 & 82.92 & 31.64 \\ 
% {\tt AIM-Prob} & 59.42 & 83.63 & 70.42 & 83.63 & 83.65 & 83.63 \\ 
% {\tt AIM-Emb} & 59.04 & 83.63 & 70.68 & 83.63 & 82.98 & 83.63 \\ \bottomrule
% \end{tabular}
% % \end{adjustbox}
% \caption{Your caption here}
% \label{tab:fusion_method}
% \end{table}


% \begin{table}[ht]
% \centering
% \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{2}{c}{Stage I} & \multicolumn{2}{c}{Stage II} & \multicolumn{2}{c}{Stage III} & \multicolumn{2}{c}{Stage IV} & \multicolumn{2}{c}{Stage V} & \multicolumn{2}{c}{Stage VI} & \multicolumn{2}{c}{Stage VII} & \multicolumn{2}{c}{Stage VIII} & \multicolumn{2}{c}{Average} \\ \cline{2-19}
%  & T & Z & T & Z & T & Z & T & Z & T & Z & T & Z & T & Z & T & Z & T & Z \\ \hline
% {\tt AVG-Prob} & 42.83 & 34.38 & 52.43 & 34.55 & 62.90 & 34.55 & 63.01 & 34.65 & 71.93 & 34.65 & 73.92 & 34.65 & 76.64 & 34.74 & 77.19 & 34.76 & 63.60 & 34.57\\ 
% {\tt AVG-Emb} & 15.87 & 6.37 & 27.67 & 16.81 & 39.14 & 22.05 & 47.66 & 24.83 & 55.70 & 24.93 & 60.58 & 25.01 & 68.47 & 25.03 & 67.89 & 25.14 & 47.87 & 21.52\\ 
% {\tt AIM-Prob} & 60.96 & 52.07 & 63.53 & 51.30 & 70.62 & 51.30 & 70.89 & 50.80 & 68.33 & 50.81 & 70.67 & 50.80 & 72.83 & 50.79 & 77.35 & 50.71 & 68.52 & 51.04\\ 
% {\tt AIM-Emb} & 60.30 & 53.61 & 63.15 & 53.68 & 70.49 & 53.84 & 70.61 & 53.78 & 66.20 & 53.82 & 69.11 & 53.82 & 72.25 & 53.82 & 72.76 & 53.77 & 67.87 & 53.77\\ 
% % Cal Tree Probe Majority & 60.78 & 53.60 & 63.49 & 53.71 & 70.55 & 53.86 & 70.63 & 53.78 & 71.24 & 53.84 & 74.40 & 53.84 & 76.46 & 53.84 & 76.98 & 53.81 & 69.32 & 53.76\\ 
% % P\_case Embedding & 60.19 & 53.62 & 63.03 & 53.67 & 70.56 & 53.84 & 70.62 &53.75 & 70.43 & 53.80 & 72.47 & 53.80 & 74.43 & 53.80 & 73.64 & 53.77 & 68.24 & 53.77\\
% % P\_case Prob & 60.93 & 52.08 & 63.57 & 51.31 & 70.66 & 51.32 & 70.76 & 50.94 & 71.89 & 50.94 & 74.62 & 50.95 & 77.15 & 50.97 & 77.95 & 50.88 & 68.56 & 51.05\\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{Your caption here}
% \label{tab:fusion_method}
% \end{table}

\begin{table}[ht]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Fusion Method} & \textbf{Target} & \textbf{Zero-shot} \\
\hline
AVG-Prob & 63.6 & 34.57 \\
\hline
AVG-Emb & 47.87 & 21.52 \\
\hline
AIM Prob & 68.52 & 51.04 \\
\hline
AIM Emb & 67.87 & 53.77 \\
\hline
\end{tabular}
\caption{Comparison of fusion operations variants}
\label{tab:fusion_methods}
\end{table}


==> tables/knn.tex <==
% \begin{table}[ht]
% \centering
% \begin{tabular}{l|cccccc}
% \hline
% Method & \multicolumn{2}{c}{Stage I (CIFAR10)} & \multicolumn{2}{c}{Stage II (SVHN)} & \multicolumn{2}{c}{Stage III (Resisc45)} \\
%  & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot \\
% \hline
% {\tt MV-KNN} & 59.64 & 83.63 & 62.09 & 83.63 & 73.64 & 83.63 \\
% {\tt AVG-KNN} & 58.99 & 83.63 & 58.70 & 83.63 & 70.95 & 83.63 \\
% {\tt WAVG-KNN} & 59.71 & 83.63 & 59.38 & 83.63 & 71.12 & 83.63 \\
% \hline
% \end{tabular}
% \caption{Your caption here}
% \label{tab:knn_prediction}
% \end{table}


% \begin{table}[ht]
% \centering
% \begin{tabular}{l|cc|cc|cc}
% \cline{2-7}
%  & \multicolumn{2}{c}{Stage I (CIFAR10)} & \multicolumn{2}{c}{Stage II (SVHN)} & \multicolumn{2}{c}{Stage III (Resisc45)} \\ \cline{2-7}
% Method & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot \\ \hline
% {\tt MV-KNN} & 59.64 & 83.63 & 62.09 & 83.63 & 73.64 & 83.63 \\ \hline
% {\tt AVG-KNN} & 58.99 & 83.63 & 58.70 & 83.63 & 70.95 & 83.63 \\ \hline
% {\tt WAVG-KNN} & 59.71 & 83.63 & 59.38 & 83.63 & 71.12 & 83.63 \\ \hline

% \end{tabular}
% \caption{Your caption here}
% \label{tab:knn_prediction}
% \end{table}


% \begin{table}[ht]
% \centering
% \begin{tabular}{l|cc|cc|cc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{2}{c}{Stage I (CIFAR10)} & \multicolumn{2}{c}{Stage II (SVHN)} & \multicolumn{2}{c}{Stage III (Resisc45)} \\ \cline{2-7}
%  & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot \\ \hline
% {\tt MV-KNN} & 59.64 & 83.63 & 62.09 & 83.63 & 73.64 & 83.63 \\ 
% {\tt AVG-KNN} & 58.99 & 83.63 & 58.70 & 83.63 & 70.95 & 83.63 \\ 
% {\tt WAVG-KNN} & 59.71 & 83.63 & 59.38 & 83.63 & 71.12 & 83.63 \\ 
% {\tt MV-TreeProbe} & 59.07 & 83.63 & 70.76 & 83.63 & 83.10 & 83.63 \\ 
% {\tt AVG-TreeProbe} & 60.32 & 83.63 & 70.66 & 83.63 & 82.99 & 83.63 \\ 
% {\tt WAVG-TreeProbe} & 60.30 & 83.63 & 70.71 & 83.63 & 83.14 & 83.63 \\ \bottomrule
% \end{tabular}
% \caption{Your caption here}
% \label{tab:knn_prediction}
% \end{table}


% \begin{table}[ht]
% \centering
% \begin{tabular}{l|c|c|c|c}
% \toprule
% Method & Stage I (CIFAR10) & Stage II (SVHN) & Stage III (Resisc45) & Average Acc. \\ \midrule
% {\tt MV-KNN} & 59.64 & 62.09 & 73.64 & 65.12 \\ 
% {\tt AVG-KNN} & 58.99 & 58.70 & 70.95 & 62.88 \\ 
% {\tt WAVG-KNN} & 59.71 & 59.38 & 71.12 & 63.40 \\ 
% {\tt MV-TreeProbe} & 59.07 & 70.76 & 83.10 & 70.98 \\ 
% {\tt AVG-TreeProbe} & 60.32 & 70.66 & 82.99 & 71.32 \\ 
% {\tt WAVG-TreeProbe} & 60.30 & 70.71 & 83.14 & 71.38 \\ \bottomrule
% \end{tabular}
% \caption{Your caption here}
% \label{tab:knn_prediction}
% \end{table}

% \begin{table}[ht]
% \centering
% \begin{tabularx}{\textwidth}{X|X|X|X|X}
% \toprule
% Method & Stage I (CIFAR10) & Stage II (SVHN) & Stage III (Resisc45) & Average \\ \midrule
% {\tt MV-KNN} & 59.64 & 62.09 & 73.64 & 65.12 \\ 
% {\tt AVG-KNN} & 58.99 & 58.70 & 70.95 & 62.88 \\ 
% {\tt WAVG-KNN} & 59.71 & 59.38 & 71.12 & 63.40 \\ 
% {\tt MV-TreeProbe} & 59.07 & 70.76 & 83.10 & 70.98 \\ 
% {\tt AVG-TreeProbe} & 60.32 & 70.66 & 82.99 & 71.32 \\ 
% {\tt WAVG-TreeProbe} & 60.30 & 70.71 & 83.14 & 71.38 \\ \bottomrule
% \end{tabularx}
% \caption{Your caption here}
% \label{tab:knn_prediction}
% \end{table}

% \begin{table}[ht]
% \centering
% \begin{tabularx}{\textwidth}{l|X|X|X|c}
% \toprule
% Method & Stage I (CIFAR10) & Stage II (SVHN) & Stage III (Resisc45) & Average \\ \midrule
% {\tt MV-KNN} & 59.64 & 62.09 & 73.64 & 65.12 \\ 
% {\tt AVG-KNN} & 58.99 & 58.70 & 70.95 & 62.88 \\ 
% {\tt WAVG-KNN} & 59.71 & 59.38 & 71.12 & 63.40 \\ 
% {\tt MV-TreeProbe} & 59.07 & 70.76 & 83.10 & 70.98 \\ 
% {\tt AVG-TreeProbe} & 60.32 & 70.66 & 82.99 & 71.32 \\ 
% {\tt WAVG-TreeProbe} & 60.30 & 70.71 & 83.14 & 71.38 \\ \bottomrule
% \end{tabularx}
% \caption{Your caption here}
% \label{tab:knn_prediction}
% \end{table}


% \begin{table}[ht]
% \centering
% \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{l|c|c|c|c}
% \toprule
% Method & Stage I (CIFAR10) & Stage II (SVHN) & Stage III (Resisc45) & Average Acc. \\ \midrule
% {\tt MV-KNN} & 59.64 & 62.09 & 73.64 & 65.12 \\ 
% {\tt AVG-KNN} & 58.99 & 58.70 & 70.95 & 62.88 \\ 
% {\tt WAVG-KNN} & 59.71 & 59.38 & 71.12 & 63.40 \\ 
% {\tt MV-TreeProbe} & 59.07 & 70.76 & 83.10 & 70.98 \\ 
% {\tt AVG-TreeProbe} & 60.32 & 70.66 & 82.99 & 71.32 \\ 
% {\tt WAVG-TreeProbe} & 60.30 & 70.71 & 83.14 & 71.38 \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{Your caption here}
% \label{tab:knn_prediction}
% \end{table}

\begin{table}[ht]
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Methods} & \textbf{Target} & \textbf{Zero-shot} \\
\hline
MV-KNN & 67.83 & 53.78 \\
\hline
AVG-KNN & 67.30 & 53.59 \\
\hline
WAVG-KNN & 67.77 & 53.83 \\
\hline
TreeProbe (MV-KNN) & 69.69 & 53.78 \\
\hline
TreeProbe (AVG-KNN) & 69.95 & 53.85 \\
\hline
TreeProbe (WAVG-KNN) & 70.00 & 53.85 \\
\hline
\end{tabular}
\caption{Comparison of KNN prediction variants}
\label{tab:knn_predictions}
\end{table}

